Fast Rates in Stochastic Online Convex Optimization by Exploiting the Curvature of Feasible Sets

In this work, we explore online convex optimization (OCO) and introduce a new condition and analysis that provides fast rates by exploiting the curvature of feasible sets. In online linear optimization, it is known that if the average gradient of loss functions exceeds a certain threshold, the curvature of feasible sets can be exploited by the follow-the-leader (FTL) algorithm to achieve a logarithmic regret. This study reveals that algorithms adaptive to the curvature of loss functions can also leverage the curvature of feasible sets. In particular, we first prove that if an optimal decision is on the boundary of a feasible set and the gradient of an underlying loss function is non-zero, then the algorithm achieves a regret bound of $O(\rho \log T)$ in stochastic environments. Here, $\rho > 0$ is the radius of the smallest sphere that includes the optimal decision and encloses the feasible set. Our approach, unlike existing ones, can work directly with convex loss functions, exploiting the curvature of loss functions simultaneously, and can achieve the logarithmic regret only with a local property of feasible sets. Additionally, the algorithm achieves an $O(\sqrt{T})$ regret even in adversarial environments, in which FTL suffers an $\Omega(T)$ regret, and achieves an $O(\rho \log T + \sqrt{C \rho \log T})$ regret in corrupted stochastic environments with corruption level $C$. Furthermore, by extending our analysis, we establish a matching regret upper bound of $O\Big(T^{\frac{q-2}{2(q-1)}} (\log T)^{\frac{q}{2(q-1)}}\Big)$ for $q$-uniformly convex feasible sets, where uniformly convex sets include strongly convex sets and $\ell_p$-balls for $p \in [2,\infty)$. This bound bridges the gap between the $O(\log T)$ bound for strongly convex sets~($q=2$) and the $O(\sqrt{T})$ bound for non-curved sets~($q\to\infty$).

==> tex_src/5_upper_old.tex <==
\section{Regret Upper Bounds}\label{sec:upper_bounds}
% ======================
\begin{wrapfigure}[9]{r}{0.4\columnwidth}
  % \begin{figure}[t]
    \centering
    \resizebox{0.33\columnwidth}{!}{%
    \input{tex_src/fig/sphere.tex}
    }
    \caption{
      The region enclosed by the black solid line is feasible set $K$ and the red dotted line $B_{\gamst}^K$ is the smallest sphere enclosing $K$ and facing $\xstar$.
    }
    \label{fig:sphere}
  % \end{figure}
  \end{wrapfigure}
  % ======================
In this section, we provide regret upper bounds that nearly match the lower bounds in \Cref{sec:lower_bounds}, by the universal online learning framework, whose regret is bounded as~\eqref{eq:uol_upper_bound}.
Note that this section works with convex loss functions.

\subsection{Stochastic Environment}
We provide logarithmic regret for stochastic environments.
Define ball $B_\gamma^K \subset \R^d$ for $\gamma > 0$ by
\begin{equation}
  B_\gamma^K
  =
  \ball\prn*{
    \xstar + \frac{1}{2 \gamma} \nabla \fcirc(\xstar) \com \,
    \frac{1}{2 \gamma} \nrm*{\nabla \fcirc(\xstar)}_2
  }
  \per 
\end{equation}
By the definition, it holds that $\xstar \in \bd(B_\gamma^K)$.
See \Cref{fig:sphere}.

\begin{remark}
The ball $B_\gamma^K$ is determined in the following manner.
We will see in the following proof that 
inequality 
$\inpr*{\nabla \fcirc(\xstar), x_t - \xstar} \geq \gamma  \nrm{x_t - \xstar}_2^2$
for some $\gamma > 0$ plays a key role in proving a logarithmic regret.
This inequality is equivalent to
$
% \begin{equation}
  \nrm*{x_t - \prn*{ \xstar + \frac{1}{2 \gamma} \nabla \fcirc(\xstar) } }_2
  \leq 
  \frac{1}{2 \gamma} \nrm*{ \nabla \fcirc(\xstar)}_2
$
% \end{equation}
and we define $B_\gamma^K$ as the set of all $x_t \in \R^d$ satisfying this inequality.
\end{remark}
Using this $B_{\gamma}^K$, we let 
$
  \gamst 
  = 
  \sup
  \set{\gamma \geq 0 \colon K \subseteq B_\gamma^K}
$.
Then, we can prove the following theorem.
\begin{theorem}\label[theorem]{thm:main}
  Consider online convex optimization in stochastic environments,
  where the optimal decision is $\xstar = \argmin_{x \in K} \fcirc(x)$.
  Suppose that $K$ is $(\rho, \xstar, \fcirc)$-sphere-enclosed
  and that $\nabla \fcirc(\xstar) \neq 0$.
  Then,
  any algorithm with bound~\eqref{eq:uol_upper_bound} achieves
  \begin{equation}
    \Reg_T 
    % &
    = 
    O \prn*{ \frac{\Csc^2}{\gamst} \log T + \Csc' \log T}
    % \nn
    % &
    =
    O \prn*{ \frac{\Csc^2 \, \rhost}{\nrm{\nabla \fcirc(\xstar)}}_2 \log T + \Csc' \log T}
    \per 
    \n
    % \\
  \end{equation}
\end{theorem}
We will see in \Cref{cor:matching_upper_bound} that this upper bound matches the lower bound in \Cref{thm:lower_bound} in the environment used to construct the lower bound.

\begin{proof}
  The regret is bounded from below by
  \begin{equation}
    \Reg_T 
    % &
    =
    \Expect{ \sumT \prx{ \fcirc(x_t) - \fcirc(\xstar) } }
    % \nn 
    % &
    \geq
    \Expect{ 
      \sumT \inpr{\nabla \fcirc(\xstar), x_t - \xstar} 
    }
    % \nn
    % &
    \geq
    \Expect{ 
      \sumT \gamst \nrm{x_t - \xstar}_2^2
    }
    \com 
    \label{eq:lb_sb}
  \end{equation}
  where the first inequality follows by the convexity of $\fcirc$, and the last inequality follows by $x_t \in K \subseteq B_{\gamst}^K$ and the definition of $\gamst$.
  By combining this inequality with inequality~\eqref{eq:uol_upper_bound},
  the regret is bounded as 
  $
  % \begin{equation}
    \Reg_T
    \leq 
    \Expect{\sumT \inpr{\nabla f_t(x_t), x_t - \xstar}}
    =
    O \prn*{
      \Csc \sqrt{\frac{\Reg_T}{\gamst} \log T}
      +
      \Csc' \log T
    }
    .
  $
  % \end{equation}
  Solving this inequation w.r.t.~$\Reg_T$, we get 
  % \begin{equation}
  $
    \Reg_T 
    =
    O \prn*{ \frac{\Csc^2}{\gamst} \log T + \Csc' \log T}
    .
    % \per 
  $
  % \end{equation}
  Observing that $\frac{1}{2 \gamst} \nrm{\nabla \fcirc(\xstar)}_2 = \rhost$, which holds from the assumption that $K$ is $(\rho, \xstar, \fcirc)$-sphere-enclosed, we complete the proof.
  \end{proof}

The advantages of the regret bound in \Cref{thm:main} compared to the existing upper bounds are the following:
  % \item  
  \one~The logarithmic regret can be achieved as long as the boundary of $K$ is curved around the optimal decision $\xstar$ or $\xstar$ in on corners (see \Cref{fig:feasible_set1}),
  while the existing analysis requires strong convexity over the entire feasible set $K$.
  % \item
  \two~While the existing analysis only considers linear loss functions,
  our approach can handle convex loss functions and thus the curvature of loss functions (\eg~strong convexity or exp-concavity) can be simultaneously exploited (see \Cref{subsec:simultaneous}).
  % \item
  \three~Even if the assumptions on loss vectors $g_1, \dots, g_T$ are not satisfied, the $O(\sqrt{T})$ regret upper bound can be achieved, while the existing approach, FTL, can suffer $\Omega(T)$ regret.

A limitation of the proposed approach is that it assumes stochastic environments.
However, our approach at least guarantees an $O(\sqrt{T})$ bound in the (fully) adversarial environments, where the growth assumption needed for FTL to achieve the fast rates is not satisfied, and as we will see in the following section, we can achieve the fast rates also in corrupted stochastic environments.

For the assumption on loss vectors, 
the existing studies consider the following assumptions on loss vectors $g_t$:
There exists $L > 0$ such that 
$\nrm{g_1 + \dots + g_T}_2 \geq t L$ for all $t \in [T]$,
or 
$g_t \leq 0$ for all $t \in [T]$.
These assumptions cannot be directly comparable with our assumption that $\nabla \fcirc(\xstar) \neq 0$.
Note that the assumption that $\inf_{x \in K} \nrm{\nabla \fcirc(x)} > 0$ is standard in the literature of offline optimization, when deriving the fast convergence rate, see~\citet{levitin66constrained,demyanov70approximate,dunn79rates} and discussion in~\citet{garber15faster} for details.

\paragraph{Tightness of regret upper bound in \Cref{thm:main}}
In the remainder of this subsection, we investigate the tightness of the regret upper bound in \Cref{thm:main}.
To see the tightness of our regret bound, 
we consider the case when $K$ is an ellipsoid.
The following proposition implies that the regret upper bound in~\Cref{thm:main} matches the lower bound in~\Cref{thm:lower_bound}.
\begin{proposition}\label[proposition]{prop:ellipsoid_mes}
  For $\lambda \in (0,1)$, let $W_\lambda$ be the ellipsoid defined in~\eqref{eq:W_lambda}.
  Then, its minimum enclosing sphere constrained so that having $(0,-\lambda)$ on it is
  % \begin{equation}
  $
    \set[\Big]{
      (x, y) \in \R^2
      \colon
      x^2 + \prn[\Big]{ y - \frac{1-\lambda^2}{\lambda} }^2
      = 
      \frac{1}{\lambda^2}
    }
    \per
    % \n
  $
  % \end{equation}
\end{proposition}
The proof of \Cref{prop:ellipsoid_mes} is deferred to \Cref{app:ellipsoid_mes}.
This result immediately implies the following matching regret upper bound.
\begin{corollary}\label[corollary]{cor:matching_upper_bound}
  Let $K$ be $W_\lambda$ and $x^* = (0, - \lambda)$.
  Under the same assumption as in \Cref{thm:main},
  in the environment considered in the construction of the lower bound in~\Cref{thm:lower_bound_growth},
  the algorithm in~\citet{wang20adaptivity} achieves
  $
  \Reg_T 
  = 
  O\prn*{
    \frac{1}{\lambda L} \log T
    +
    G D \log T
  }
  .
  $
\end{corollary}
We can see that this upper bound matches the lower bound in~\Cref{thm:lower_bound} up to the additive $G D \log T$ factor.
\begin{proof}
  From \Cref{prop:ellipsoid_mes} and the fact that Euclidean ball with radius $r$ is $1/r$ strongly convex w.r.t.~$\nrm{\cdot}_2$, we have $\rho = 1/\lambda$.
  This proposition combined with~\Cref{thm:main} immediately gives the desired bound.
\end{proof}
The upper bound in \Cref{thm:main} is applicable when $K$ is a polytope.
We will see that our approach work also in the corrupted stochastic environment in \Cref{subsec:corruption},
and to our knowledge,
this is the first upper bound that achieves fast rates when the feasible set is a polytope in non-stochastic environments. 
A further discussion when $K$ is a polytope can be found in \Cref{app:polytope}. 


\subsection{Corrupted Stochastic Environments}\label{subsec:corruption}
Another advantage of our approach is that it can achieve nearly optimal regret upper bounds even in corrupted stochastic environments.
for this $\tilde{B}_\gamma^K$, we let 
$    
\gamtilstar = \sup
\set{\gamma \geq 0  \colon K \subseteq \widetilde{B}_\gamma^K}.
$
For $\gamma > 0$, we define ball $\widetilde{B}_\gamma^K \subset \R^d$ by
$
% \begin{equation}
  \widetilde{B}_\gamma^K
  =
  \ball\prn[\big]{
    \xtilstar + \frac{1}{2 \gamma} \nabla \ftilcirc(\xtilstar) \com \,
    \frac{1}{2 \gamma} \nrm[\big]{\nabla \ftilcirc(\xtilstar)}_2
  }
  \com 
  % \n
$
% \end{equation}
which is defined in the same manner as $B_\gamma^K$.
Then, we can prove the following regret upper bound.
\begin{theorem}\label[theorem]{thm:main_corruption}
  Consider online convex optimization in corrupted stochastic environments with corruption level at most $C$, where
  $\xtilstar = \argmin_{x \in K} \ftilcirc(x)$. %  is on the boundary of $K$,
  Suppose $K$ is $(\rho, \xtilstar, \ftilcirc)$-sphere enclosed 
  and $\nabla \ftilcirc(\xtilstar) \neq 0$.
  Then, any algorithm with bound~\eqref{eq:uol_upper_bound} achieves
  \begin{equation}
    % &
    \Reg_T % (\xstar) 
    = 
    O \prn*{ \frac{\Csc^2}{\gamtilstar} \log T 
      +
      \sqrt{
        \frac{C \Csc^2}{\gamtilstar} \log T 
      }
      +
      \Csc' \log T
    }
    % \nn
    % &
    =
    O \prn*{ 
      \frac{\Csc^2 \, \rhost}{\nrm{\nabla \ftilcirc(\xtilstar)}}_2 \log T 
      +
      \sqrt{
        \frac{ C \Csc^2 \, \rhost}{\nrm{\nabla \ftilcirc(\xtilstar)}}_2 \log T 
      }
      + 
      \Csc' \log T
    }
    \per 
    \n
  \end{equation}
\end{theorem}
The proof of \Cref{thm:main_corruption} can be found in \Cref{app:corruption}.
We can observe that this upper bound matches the lower bound in \Cref{thm:lower_bound_corrupt} up to logarithmic factors, considering the environment to prove the lower bound.
It is worth mentioning that all upper bounds provided in this paper can be extended following the same line as the proof of \Cref{thm:main_corruption}.



\subsection{Exploiting the Curvature of Loss Functions and Feasible Sets Simultaneously}\label{subsec:simultaneous}
One of the advantages of directly solving OCO over reducing to OLO is that we can obtain upper bounds that can simultaneously exploit the curvature of feasible sets and loss functions:
\begin{theorem}\label[theorem]{thm:main_sim_curvature}
Suppose that the same assumption as in \Cref{thm:main} holds.
If $f_1, \dots, f_T$ are $\alpha$-strongly convex w.r.t.~a norm $\nrm{\cdot}$, then
% \begin{equation}
$
  \Reg_T
  = 
  O \prn*{ \frac{\Csc^2}{\gamst + \alpha / \xi} \log T + \Csc' \log T}
  .
  % \com 
  % \n 
$
% \end{equation}
If $f_1, \dots, f_T$ are $\beta$-exp-concave, then
% \begin{equation}
$
  \Reg_T
  = 
  O\prn*{
    \min \set*{
      \frac{\Csc^2}{\gamst}
      \com
      \frac{\Cec^2}{\beta' + \gamst / G^2}
    }
    \log T
    +
    \max\set*{\Csc', \Cec'} \log T
  }
$
  % \n
% \end{equation}
for $\beta' \leq \frac12 \min\set*{\frac{1}{4 G D}, \beta}$.
% Here  
% $
% \gamst 
% = 
% \sup
% \set{\gamma \geq 0  \colon K \subseteq B_\gamma^K}
% $
% satisfies $\rho = \frac{1}{2\gamst} \nrm{\nabla \fcirc(\xstar)}_2$.
\end{theorem}
The proof can be found in Appendix~\ref{app:sim_curvature}.
\Cref{thm:main_sim_curvature} implies that one can simultaneously exploit the curvature of feasible sets and loss functions.
Note that the similar analysis is possible for corrupted stochastic environments. 


\subsection{Extending Analysis to Uniformly Convex Sets}\label{subsec:unif_convex}
Here, we prove that a regret upper bound smaller than $O(\sqrt{T})$ can be achieved when $K$ is uniformly convex.
This can be proven by essentially a similar argument using the idea of exploiting the lower bound, as done in the proof for sphere-enclosed sets. 
\begin{definition}\label[definition]{def:uniformly_convex}
  A convex body $K$ is $(\kappa, q)$-uniformly convex w.r.t.~a norm $\nrm{\cdot}$ (or $q$-uniformly convex)
  if for any $ x, y \in K $ and any $\theta \in [0,1]$, it holds that
  $
    \theta x + (1 - \theta) y 
    +
    \theta (1 - \theta)
    \frac{\kappa}{2}
    \nrm{ x - y }^q
    \cdot \ball_{\nrm{\cdot}}
    \subseteq 
    K \per    
  $
\end{definition}
For example, $\ell_p$-balls are $(1/p, p)$-uniformly convex w.r.t.~$\nrm{\cdot}_p$ for $p \geq 2$~\citep[Theorem 2]{hanner56uniform},
and $p$-Schatten balls are $(1/p ,p)$-uniformly convex w.r.t.~the Schatten norm $\nrm{\cdot}_{S(p)}$ 
(See \citet{kerdreux21projection} for the connection between the uniform convexity of a normed space and the uniform convexity of sets.)
Note that $(\kappa, 2)$-uniformly convex set is $\kappa$-strongly convex.
For the uniformly convex feasible sets, we can prove the following theorem.
\begin{theorem}\label[theorem]{thm:main_uniform_cvx}
  Consider online convex optimization in stochastic environments,
  where the optimal decision is $\xstar = \argmin_{x \in K} \fcirc(x)$.
  Suppose that $K$ is $(\kappa, q)$-uniformly convex w.r.t.~a norm $\nrm{\cdot}$ for some $q \geq 2$
  and that $\nabla \fcirc(\xstar) \neq 0$.
  Then, any algorithm with bound~\eqref{eq:uol_upper_bound} achieves
  \begin{equation}
    \Reg_T % (\xstar) 
    % &
    % \leq 
    =
    \prn*{ 
      \frac
        { \prn*{ \xi \Csc }^{\frac{q}{q-1}} }
        {
          \prn*{
          q
          \kappa
          \nrm{ \nabla \fcirc(\xstar) }_\star
          }^{\frac{1}{q-1}}
        }
        T^{\frac{q-2}{2(q-1)}}
        \prn*{ \log T }^{\frac{q}{2(q-1)}}
        + 
        \Csc' \log T
    }
    \per 
  \end{equation}
  In particular,
  when $K$ is $\lambda$-strongly convex w.r.t.~a norm $\nrm{\cdot}$,
  $
    \Reg_T
    = 
    O \prn*{ 
      \frac
        { \xi \Csc }
        {
          \lambda
          \nrm{ \nabla \fcirc(\xstar) }_\star
        } 
        \log T
        + 
        \Csc' \log T
    }
    \per 
  $  
\end{theorem}
The dependence on $T$ in this bound is $O\prn*{T^{\frac{q-2}{2(q-1)}} \prn*{ \log T }^{\frac{q}{2(q-1)}}}$,
which becomes $O(\log T)$ when $q = 2$ and $\tilde{O}(\sqrt{T})$ when $q\to\infty$, and thus interpolates between the bound over the strongly convex sets and non-curved feasible sets.
This is strictly better than the $O\prn*{T^{\frac{q-2}{q-1}}}$ bound in~\citet{kerdreux21projection}; their regret upper bound is better than $O(\sqrt{T})$ only when $q \in (2, 3)$.
For example, when $K$ is $\ell_p$-ball, 
by $\nrm{x}_2 \leq d^{\frac12 - \frac1p} \nrm{x}_p$ for any $x \in \R^d$ and $p > 2$, the regret is bounded as
$
  \Reg_T
  = 
  O \prn[\bigg]{ 
    \frac
      { \prn*{ \xi \Csc }^{\frac{p}{p-1}} d^{\frac{p-2}{2(p-1)}}}
      {
        \prn*{
        \nrm{ \nabla \fcirc(\xstar) }_\star
        }^{\frac{1}{p-1}}
      } 
      T^{\frac{p-2}{2(p-1)}}
      \prn*{ \log T }^{\frac{p}{2(p-1)}}
      + 
      \Csc' \log T
  }
  . 
$
Note that the similar analysis is possible for corrupted stochastic environments.
\begin{proof}
From $\xstar = \argmin_{x \in K} \fcirc(x)$  and the first-order optimality condition,
$ \inpr{\nabla \fcirc(\xstar), x - \xstar} \geq 0 $,
which implies that $\xstar = \argmin_{x \in K} \inpr{\nabla \fcirc(\xstar), x}$.
Hence, combining this with \citet[Lemma 2.1]{kerdreux21linear} and that $K$ is $(\kappa, q)$-uniformly convex w.r.t.~a norm $\nrm{\cdot}$,
it holds that
$
% \begin{equation}
  \inpr{ \nabla \fcirc(\xstar), x - \xstar}
  \geq 
  \frac{\kappa}{2} \nrm{x - \xstar}^q \cdot \nrm{\nabla \fcirc(\xstar)}_\star
  % \quad
  % \mbox{for all}
  % \,
  % x \in K
  % \per
$
for all $x \in K$.
% \end{equation}
Using this inequality,
\begin{align}
  \Reg_T % (\xstar) 
  &
  =
  \Expect{ \sumT \prx{ \fcirc(x_t) - \fcirc(\xstar) } }
  % \nn 
  % &
  \geq
  \Expect{ 
    \sumT \inpr{\nabla \fcirc(\xstar), x_t - \xstar} 
  }
  \nn
  &
  \geq
  \frac{\kappa}{2} \nrm{\nabla \fcirc(\xstar)}_\star
  \cdot 
  \Expect{
    \sumT 
    \nrm{x - \xstar}^q 
  }
  % \nn 
  % &
  \geq 
  \frac{\kappa}{2 \xi^q} \nrm{\nabla \fcirc(\xstar)}_\star
  \cdot 
  \Expect{
    \sumT 
    \nrm{x - \xstar}_2^q 
  }
  \nn 
  &
  \geq 
  \frac{\kappa}{2 \xi^q} \nrm{\nabla \fcirc(\xstar)}_\star
  \,
  T^{1 - \frac{q}{2}}
  % \cdot
  \prn*{ 
  \Expect{
    \sumT 
    \nrm{x - \xstar}_2^2
  }
  }^{q/2}
  \com 
  \label{eq:unif_lb}
\end{align}
where the first inequality follows by the convexity of $\fcirc$, 
the second inequality by $\nrm{x}_2 \leq \xi \nrm{x}$ for any $x \in \R^d$,
and the last inequality by Jensen's inequality and the fact that $x \mapsto x^{q/2}$ is convex for $q \geq 2$.
Combining~\eqref{eq:uol_upper_bound} and~\eqref{eq:unif_lb},
we can bound the regret as
\begin{align}
  &
  \Reg_T
  = 
  2 \Reg_T - \Reg_T
  \nn
  &= 
  O \prn*{ 
    % 2
    \Csc 
    \sqrt{
      \Expect{ \sumT \nrm{x_t - \xstar}_2^2 } \log T
    }
    -
    \frac{\kappa}{\xi^q} \nrm{\nabla \fcirc(\xstar)}_\star
    \,
    T^{1 - \frac{q}{2}}
    \prn*{ 
    \Expect{
      \sumT 
      \nrm{x - \xstar}_2^2
    }
    }^{q/2}
    + 
    \Csc' \log T 
  }
  \nn
  &= 
  O \prn*{ 
    \frac
      { \prn*{ \xi \Csc }^{\frac{q}{q-1}} }
      {
        \prn*{
        q
        \kappa
        \nrm{ \nabla \fcirc(\xstar) }_\star
        }^{\frac{1}{q-1}}
      } 
      T^{\frac{q-2}{2(q-1)}}
      \prn*{ \log T }^{\frac{q}{2(q-1)}}
      + 
      \Csc' \log T
  } 
  \com 
\end{align}
where in the last line we used the inequality 
$ a \sqrt{x} - b x^{q/2} \leq \frac{a^{\frac{q}{q-1}}}{(q b)^{\frac{1}{q-1}}}$ that holds for $a, b, x > 0$ and $q \geq 2$.
This completes the proof.
\end{proof}














